Statistical Analysis of the Dearth of Super-eccentric Jupiters in the Kepler Sample

Hot Jupiters may have formed in situ, or been delivered to their observed short periods through one of two categories of migration mechanisms: disk migration or high-eccentricity migration. If hot Jupiters were delivered by high-eccentricity migration, we would expect to observe some "super-eccentric" Jupiters in the process of migrating. We update a prediction for the number of super-eccentric Jupiters we would expect to observe in the Kepler sample if all hot Jupiters migrated through high-eccentricity migration and estimate the true number observed by Kepler. We find that the observations fail to match the prediction from high-eccentricity migration with 94.3% confidence and show that high-eccentricity migration can account for at most ~62% of the hot Jupiters discovered by Kepler.

==> candidate_table.tex <==
\begin{scriptsize}
%\begin{landscape}
\begin{ThreePartTable}
\begin{longtable}[ht]{l l l l l l l l l}
\caption{Warm Jupiter planet candidate sample}
\label{tab:candidates}

\\
\toprule
KIC & KOI & Kepler & Period & $\rho_{\rm{circ}}/\rho_*$\tnote{2} & Radius & Weight\tnote{3} & Estimated $e$\tnote{4} & Probability\tnote{5} \\ number\tnote{1} & number & number & (days) & & ($R_{\earth}$) & & & \\ \midrule
\endfirsthead

\multicolumn{9}{l}{{\tablename\ \thetable{} -- \emph{continued from previous page}}}\\
\toprule
KIC & KOI & Kepler & Period & $\rho_{\rm{circ}}/\rho_*$\tnote{2} & Radius & Weight\tnote{3} & Estimated $e$\tnote{4} & Probability\tnote{5} \\ number\tnote{1} & number & number & (days) & & ($R_{\earth}$) & & & \\  \midrule
\endhead

\bottomrule
\\
\multicolumn{8}{l}{{\emph{\tablename\ \thetable{} continued on next page}}} \\
\endfoot
\bottomrule
\endlastfoot

%2853093 & Kepler-767 b & 161.53 & 90.97 & $8.19^{+1.36}_{-1.23}$ & 1.000 & $0.91_{-0.07}^{+0.05}$ & 30.2\%\\[2pt]
3534076 & 1209.01 & - & 272.09 & 23.49 & $5.95^{+2.67}_{-0.53}$ & 0.028 & $0.18_{-0.18}^{+0.51}$ & 1.9\%\\[2pt]
3942446 & 1193.01 & - & 119.06 & 20.46 & $10.4^{+2.82}_{-1.89}$ & 0.619 & $0_{-0}^{+0.79}$ & 4.2\%\\[2pt]
4155328 & 1335.01 & 820b & 127.83 & 3.29 & $9.46^{+1.56}_{-2.14}$ & 0.727 & $0.43_{-0.43}^{+0.29}$ & 4.0\%\\[2pt]
4544670 & 815.01 & - & 35.74 & 59.87 & $7.61^{+1.72}_{-0.91}$ & 0.996 & $0.46_{-0.46}^{+0.27}$ & 0.3\%\\[2pt]
4566848 & 5071.01 & - & 180.41 & 13.57 & $8.86^{+2.60}_{-0.86}$ & 0.099 & $0\pm0$ & 0.9\%\\[2pt]
4918309 & 1582.01 & - & 186.44 & 1.31 & $11.32^{+1.80}_{-3.35}$ & 0.890 & $0.21_{-0.18}^{+0.39}$ & 1.6\%\\[2pt]
5184584 & 1564.01 & 891b & 53.45 & 10.96 & $5.82^{+1.49}_{-0.50}$ & 1.000 & $0.70_{-0.14}^{+0.17}$ & 3.3\%\\[2pt]
5966810 & 3909.01 & - & 247.89 & 0.29 & $4.74\pm0.87$ & 0.001 & $0\pm0$ & 0.1\%\\[2pt]
6471021 & 372.01 & 539b & 125.63 & 0.93 & $10.02^{+1.47}_{-1.33}$ & 0.792 & $0.05_{-0.05}^{+0.32}$ & 1.0\%\\[2pt]
6504954 & 1790.01 & 952b & 130.35 & 3.46 & $7.70^{+2.53}_{-0.84}$ & 0.717 & $0.44_{-0.44}^{+0.31}$ & 3.1\%\\[2pt]
6766634 & 1375.01 & 1746b & 321.21 & 16.71 & $7.25^{+1.16}_{-1.17}$ & 0.989 & $0.79_{-0.10}^{+0.12}$ & 5.4\%\\[2pt]
6937692 & 513.01 & 584b & 35.18 & 0.05 & $4.17^{+1.24}_{-0.54}$ & 0.005 & $0\pm0$ & 0.1\%\\[2pt]
7211141 & 1355.01 & 827b & 51.93 & 7.26 & $8.49^{+1.40}_{-1.86}$ & 0.305 & $0_{-0}^+{0.66}$ & 1.2\%\\[2pt]
7619236 & 682.01 & - & 562.70 & 1.63 & $10.90^{+1.96}_{-1.72}$ & 0.992 & $0.31_{-0.14}^{+0.41}$ & 1.1\%\\[2pt]
7811397 & 1477.01 & - & 169.50 & 1.07 & $9.06^{+0.90}_{-0.28}$ & 1.000 & $0.13_{-0.10}^{+0.39}$ & 2.2\%\\[2pt]
7951018 & 1553.0 & 890b & 52.76 & 3.23 & $8.76^{+2.91}_{-0.97}$ & 1.000 & $0.53_{-0.14}^{+0.27}$ & 2.1\%\\[2pt]
7984047 & 1552.01 & - & 77.63 & 4.69 & $9.40^{+0.67}_{-0.92}$ & 1.000 & $0.60_{-0.12}^{+0.27}$ & 5.0\%\\[2pt]
%8559644 & Kepler-953 b & 224.78 & 0.31 & $4.55^{+0.73}_{-0.45}$ & 0.005 & $0\pm0$ & \\[2pt] might not be unstable
8672910 & 918.01 & 725b & 39.64 & 0.73 & $10.98^{+0.72}_{-0.99}$ & 1.000 & $0.24_{-0.13}^{+0.45}$ & 0.4\%\\[2pt]
8686373 & 4066.01 & 1936b & 126.56 & 0.05 & $4.59^{+1.44}_{-1.43}$ & 0.014 & $0\pm0$ & 0.1\%\\[2pt]
8813698 & 1268.01 & - & 268.94 & 5.48 & $13.57^{+2.30}_{-2.31}$ & 1.000 & $0.66_{-0.12}^{+0.20}$ & 4.5\%\\[2pt]
8827930 & 3801.01 & - & 288.31 & 15.47 & $13.21^{+2.07}_{-2.30}$ & 1.000 & $0.77_{-0.10}^{+0.15}$ & 6.4\%\\[2pt]
9025971 & 3680.01 & 1657b & 141.23 & 3.60 & $11.49^{+1.66}_{-1.21}$ & 1.000 & $0.55_{-0.13}^{+0.27}$ & 4.7\%\\[2pt]
9147029 & 5626.01 & - & 397.50 & 1.54 & $6.57^{+3.9}_{-0.91}$ & 0.001 & $0\pm0$ & 0.1\%\\[2pt]
9425139 & 1411.01 & - & 305.08 & 3.53 & $7.82^{+1.25}_{-0.84}$ & 0.326 & $0_{-0}^{+0.58}$ & 0.8\%\\[2pt]
9480535 & 3901.01 & 1527b & 160.13 & 0.10 & $6.67^{+1.19}_{-1.47}$ & 0.013 & $0\pm0$ & 0.1\%\\[2pt]
9512981 & 1466.01 & - & 281.56 & 1.86 & $10.83^{+0.37}_{-0.70}$ & 1.000 & $0.36_{-0.14}^{+0.37}$ & 2.8\%\\[2pt]
9958387 & 2677.01 & - & 237.79 & 0.45 & $9.91^{+1.84}_{-4.28}$ & 0.984 & $0.43_{-0.18}^{+0.33}$ & 2.4\%\\[2pt]
10265602 & 2689.01 & - & 165.34 & 14.01 & $6.98^{+1.53}_{-0.82}$ & 0.983 & $0.69^{+0.19}_{-0.69}$ & 6.1\%\\[2pt]
10656508 & 211.01 & - & 124.04 & 22.21 & $11.13\pm1.80$ & 1.000 & $0.82_{-0.06}^{+0.11}$ & 15.8\%\\[2pt]
10795103 & 3683.01 & 1515b & 214.31 & 1.06 & $9.17^{+1.64}_{-0.93}$ & 1.000 & $0.11_{-0.09}^{+0.41}$ & 1.2\%\\[2pt]
11027624 & 1439.01 & 849b & 394.62 & 0.87 & $7.79^{+1.27}_{-1.90}$ & 0.832 & $0.12_{-0.12}^{+0.41}$ & 1.4\%\\[2pt]
11036168 & 5855.01 & - & 217.79 & 0.70 & $6.15^{+0.96}_{-1.17}$ & 0.025 & $0\pm0$ & 0.1\%\\[2pt]
11075279 & 1431.01 & - & 345.16 & 1.12 & $7.79^{+1.13}_{-0.36}$ & 0.586 & $0.02_{-0.02}^{+0.28}$ & 0.8\%\\[2pt]
11189311 & 3220.01 & 1442b & 81.42 & 0.01 & $4.63^{+0.87}_{-0.44}$ & 0.004 & $0\pm0$ & 0.2\%\\[2pt]
11449844 & 125.01 & 468b & 38.48 & 1.76 & $13.26^{+1.78}_{-0.59}$ & 0.962 & $0.33_{-0.14}^{+0.39}$ & 0.8\%\\[2pt]
%12365184 & Kepler-419 b & 69.73 & & $11.65\pm2.12$ & N/A & N/A & N/A \\[2pt]
12406749 & 1476.01 & 1752b & 56.36 & 0.04 & $5.04^{+0.96}_{-0.52}$ & 0.010 & $0\pm0$ & 0.1\%\\[2pt]
	 
\end{longtable}

\begin{tablenotes}
\item[1] Kepler Input Catalog number of host star
\item[2] Mean $\rho_{\rm{circ}}$ over mean $\rho_*$
\item[3] Fraction of planetary radius posterior that falls within 8-22$R_{\earth}$
\item[4] See Section \ref{model}
\item[5] Posterior probability of $e>0.9$ and $2.8<P_{\rm{final}}<10$ days
\end{tablenotes}

\end{ThreePartTable}

%\end{landscape}
\end{scriptsize}
